Modular coinduction up-to for higher-order languages via first-order transition systems

The bisimulation proof method can be enhanced by employing `bisimulations up-to' techniques. A comprehensive theory of such enhancements has been developed for first-order (i.e., CCS-like) labelled transition systems (LTSs) and bisimilarity, based on abstract fixed-point theory and compatible functions. We transport this theory onto languages whose bisimilarity and LTS go beyond those of first-order models. The approach consists in exhibiting fully abstract translations of the more sophisticated LTSs and bisimilarities onto the first-order ones. This allows us to reuse directly the large corpus of up-to techniques that are available on first-order LTSs. The only ingredient that has to be manually supplied is the compatibility of basic up-to techniques that are specific to the new languages. We investigate the method on the pi-calculus, the lambda-calculus, and a (call-by-value) lambda-calculus with references.

==> Makefile <==
f=fo

all: ${f}.pdf responseletter.pdf

# rubber -d

${f}.pdf: ${f}.tex davidemacro.tex fo.tex implambda.tex intro.tex lambda.tex pi.tex references.bib conclusions.tex  Makefile
	rubber -d ${f}.tex
# pdflatex ${f}.tex
# bibtex ${f}.aux
# pdflatex ${f}.tex
# pdflatex ${f}.tex

responseletter.pdf: responseletter.tex Makefile
	rubber -d responseletter.tex

clean:
	rm -f ${f}.aux ${f}.bbl ${f}.blg ${f}.log ${f}.pdf

journal.zip: conclusions.tex davidemacro.tex fo.tex fo.bbl implambda.tex intro.tex lambda.tex pi.tex Makefile pi.tex references.bib utf8-aliases.inc
	zip journal.zip \
             conclusions.tex davidemacro.tex fo.tex fo.bbl implambda.tex intro.tex lambda.tex pi.tex Makefile pi.tex references.bib utf8-aliases.inc

